Towards Interpretable Framework for Neural Audio Codecs via Sparse Autoencoders: A Case Study on Accent Information

Neural Audio Codecs (NACs) are widely adopted in modern speech systems, yet how they encode linguistic and paralinguistic information remains unclear. Improving the interpretability of NAC representations is critical for understanding and deploying them in sensitive applications. Hence, we employ Sparse Autoencoders (SAEs) to decompose dense NAC representations into sparse, interpretable activations. In this work, we focus on a challenging paralinguistic attribute-accent-and propose a framework to quantify NAC interpretability. We evaluate four NAC models under 16 SAE configurations using a relative performance index. Our results show that DAC and SpeechTokenizer achieve the highest interpretability. We further reveal that acoustic-oriented NACs encode accent information primarily in activation magnitudes of sparse representations, whereas phonetic-oriented NACs rely more on activation positions, and that low-bitrate EnCodec variants show higher interpretability.

==> tables/US_Other_Main.tex <==
\begin{tabular}{ccccccccc}
\toprule
& \multicolumn{4}{c}{Acoustic NACs} & \multicolumn{4}{c}{Phonetic NACs} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
$D_\text{z}/D_\text{d}$
& \multicolumn{2}{c}{EnCodec} & \multicolumn{2}{c}{DAC}
& \multicolumn{2}{c}{Mimi} & \multicolumn{2}{c}{SpeechTokenizer} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
& Acc (\%) & F1 (\%) & Acc (\%) & F1 (\%) & Acc (\%) & F1 (\%) & Acc (\%) & F1 (\%) \\
\midrule

\multicolumn{9}{l}{\textbf{Reference}}\\
1  & 70.81$\pm$0.01 & 66.42$\pm$0.03 & 69.86$\pm$0.03 & 66.28$\pm$0.08 & 79.90$\pm$0.00 & 78.57$\pm$0.00 & 78.83$\pm$0.02 & 77.28$\pm$0.03 \\
\midrule

\multicolumn{9}{l}{\textbf{Relative Sparsity $\mathbf{s}=5\%$}}\\
2  & 63.45$\pm$0.05 & 50.68$\pm$0.04 & 73.09$\pm$0.11 & 69.84$\pm$0.37 & 64.65$\pm$0.01 & 53.53$\pm$0.01 & 63.71$\pm$0.02 & 51.48$\pm$0.11 \\
5  & 63.95$\pm$0.02 & 50.95$\pm$0.09 & 73.23$\pm$0.01 & 69.83$\pm$0.13 & 64.22$\pm$0.00 & 51.69$\pm$0.00 & 63.60$\pm$0.49 & 51.64$\pm$1.75 \\
10 & 65.80$\pm$0.11 & 57.03$\pm$0.39 & 71.10$\pm$0.01 & 67.53$\pm$0.02 & 64.66$\pm$0.00 & 53.40$\pm$0.00 & 63.63$\pm$0.05 & 51.30$\pm$0.58 \\
20 & 64.73$\pm$0.01 & 54.18$\pm$0.03 & 70.25$\pm$0.01 & 66.34$\pm$0.01 & 65.00$\pm$0.01 & 54.65$\pm$0.02 & 64.69$\pm$0.18 & 54.30$\pm$0.61 \\
\midrule

\multicolumn{9}{l}{\textbf{Relative Sparsity $\mathbf{s}=10\%$}}\\
2  & 65.94$\pm$0.01 & 58.26$\pm$0.12 & 70.42$\pm$1.30 & 65.56$\pm$3.07 & 63.87$\pm$0.01 & 52.97$\pm$1.40 & 65.44$\pm$0.25 & 57.55$\pm$1.30 \\
5  & 65.86$\pm$0.02 & 56.01$\pm$0.18 & 73.34$\pm$0.12 & 70.28$\pm$0.46 & 63.75$\pm$0.00 & 50.20$\pm$0.00 & 64.89$\pm$0.20 & 55.07$\pm$1.95 \\
10 & 67.86$\pm$0.01 & 61.03$\pm$0.05 & 69.53$\pm$0.36 & 65.16$\pm$0.84 & 63.71$\pm$0.00 & 49.85$\pm$0.00 & 64.18$\pm$0.08 & 53.19$\pm$2.63 \\
20 & 64.14$\pm$0.02 & 54.50$\pm$0.15 & 66.45$\pm$0.04 & 60.13$\pm$0.29 & 63.82$\pm$0.00 & 52.48$\pm$0.00 & 63.34$\pm$0.15 & 53.45$\pm$0.75 \\
\midrule

\multicolumn{9}{l}{\textbf{Relative Sparsity $\mathbf{s}=25\%$}}\\
2  & 65.93$\pm$0.09 & 56.99$\pm$0.24 & 68.50$\pm$0.29 & 63.88$\pm$1.12 & 64.16$\pm$0.01 & 52.19$\pm$0.03 & 63.55$\pm$2.98 & 55.01$\pm$1.73 \\
5  & 67.07$\pm$0.01 & 60.24$\pm$0.03 & 71.48$\pm$0.29 & 67.83$\pm$0.66 & 63.72$\pm$0.01 & 51.67$\pm$0.01 & 64.26$\pm$0.66 & 57.94$\pm$5.21 \\
10 & 63.40$\pm$0.01 & 54.38$\pm$0.04 & 70.33$\pm$0.09 & 66.29$\pm$0.21 & 63.70$\pm$0.01 & 55.52$\pm$0.01 & 67.51$\pm$0.45 & 60.71$\pm$1.35 \\
20 & 67.82$\pm$0.01 & 61.60$\pm$0.03 & 70.55$\pm$0.15 & 65.92$\pm$0.31 & 64.48$\pm$0.00 & 54.67$\pm$0.01 & 65.80$\pm$0.48 & 59.42$\pm$2.82 \\
\midrule

\multicolumn{9}{l}{\textbf{Relative Sparsity $\mathbf{s}=50\%$}}\\
2  & 67.83$\pm$0.01 & 61.81$\pm$0.08 & 68.19$\pm$0.15 & 62.62$\pm$0.74 & 63.32$\pm$0.04 & 52.00$\pm$0.10 & 66.11$\pm$0.38 & 59.65$\pm$3.04 \\
5  & 62.76$\pm$0.01 & 54.36$\pm$0.01 & 70.44$\pm$0.09 & 66.51$\pm$0.40 & 64.62$\pm$0.01 & 52.78$\pm$0.04 & 64.91$\pm$0.51 & 56.14$\pm$2.57 \\
10 & 65.66$\pm$0.00 & 58.76$\pm$0.00 & 67.54$\pm$0.18 & 62.33$\pm$0.84 & 66.65$\pm$0.01 & 59.28$\pm$0.05 & 63.26$\pm$1.10 & 58.65$\pm$3.28 \\
20 & 65.69$\pm$0.00 & 57.98$\pm$0.00 & 69.86$\pm$0.29 & 65.49$\pm$0.77 & 68.33$\pm$0.03 & 61.66$\pm$0.06 & 64.88$\pm$0.59 & 57.33$\pm$2.25 \\
\bottomrule
\end{tabular}


==> tables/US_UK_Main.tex <==
% Requires in preamble:
% \usepackage{booktabs}


\begin{tabular}{c c c c c c c c c}
\toprule
& \multicolumn{4}{c}{\textbf{Acoustic NACs}} & \multicolumn{4}{c}{\textbf{Phonetic NACs}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
\textbf{$\frac{D_\text{z}}{D_\text{d}}$}
& \multicolumn{2}{c}{\textbf{EnCodec}} & \multicolumn{2}{c}{\textbf{DAC}}
& \multicolumn{2}{c}{\textbf{Mimi}} & \multicolumn{2}{c}{\textbf{SpeechTokenizer}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
& Acc (\%) & F1 (\%) & Acc (\%) & F1 (\%) & Acc (\%) & F1 (\%) & Acc (\%) & F1 (\%) \\
\midrule

\multicolumn{9}{l}{\textbf{Reference}}\\
1  & 84.31$\pm$0.02 & 83.72$\pm$0.02 & 84.21$\pm$0.01 & 83.53$\pm$0.03 & 90.70$\pm$0.00 & 90.59$\pm$0.00 & 93.47$\pm$0.01 & 93.45$\pm$0.01 \\
\midrule

\multicolumn{9}{l}{\textbf{Relative Sparsity $\mathbf{s}=5\%$}}\\
2  & 64.72$\pm$0.27 & 59.52$\pm$0.19 & 79.63$\pm$0.01 & 78.88$\pm$0.02 & 72.13$\pm$0.00 & 69.20$\pm$0.00 & 75.97$\pm$0.15 & 74.18$\pm$0.25 \\
5  & 67.43$\pm$0.09 & 62.50$\pm$0.01 & 81.11$\pm$0.05 & 80.54$\pm$0.07 & 79.58$\pm$0.00 & 78.66$\pm$0.00 & 71.47$\pm$0.11 & 70.35$\pm$0.43 \\
10 & 68.19$\pm$0.05 & 64.62$\pm$0.07 & 80.33$\pm$0.09 & 79.69$\pm$0.02 & 74.62$\pm$0.00 & 71.81$\pm$0.00 & 74.12$\pm$1.86 & 73.67$\pm$1.09 \\
20 & 70.86$\pm$0.08 & 67.97$\pm$0.02 & 81.50$\pm$0.01 & 80.79$\pm$0.03 & 74.98$\pm$0.00 & 73.11$\pm$0.00 & 74.12$\pm$0.34 & 72.18$\pm$0.08 \\
\midrule

\multicolumn{9}{l}{\textbf{Relative Sparsity $\mathbf{s}=10\%$}}\\
2  & 66.62$\pm$0.08 & 61.93$\pm$0.09 & 80.37$\pm$0.06 & 79.14$\pm$0.17 & 77.55$\pm$0.00 & 76.48$\pm$0.00 & 74.40$\pm$0.10 & 71.86$\pm$0.27 \\
5  & 71.40$\pm$0.14 & 70.05$\pm$0.02 & 79.55$\pm$0.06 & 78.63$\pm$0.13 & 77.57$\pm$0.00 & 76.45$\pm$0.00 & 71.41$\pm$0.50 & 67.90$\pm$0.30 \\
10 & 70.49$\pm$0.02 & 69.13$\pm$0.05 & 79.77$\pm$0.02 & 78.77$\pm$0.08 & 73.02$\pm$0.00 & 70.19$\pm$0.00 & 75.82$\pm$0.53 & 74.11$\pm$0.05 \\
20 & 70.32$\pm$0.01 & 68.68$\pm$0.01 & 79.78$\pm$0.06 & 78.59$\pm$0.13 & 75.53$\pm$0.00 & 73.54$\pm$0.00 & 78.44$\pm$0.06 & 76.95$\pm$0.43 \\
\midrule

\multicolumn{9}{l}{\textbf{Relative Sparsity $\mathbf{s}=25\%$}}\\
2  & 79.24$\pm$0.01 & 78.38$\pm$0.01 & 78.98$\pm$0.01 & 77.98$\pm$0.06 & 71.32$\pm$0.02 & 68.60$\pm$0.05 & 81.55$\pm$0.07 & 80.84$\pm$0.23 \\
5  & 73.38$\pm$0.01 & 71.58$\pm$0.01 & 80.12$\pm$0.03 & 79.24$\pm$0.11 & 72.40$\pm$0.02 & 70.93$\pm$0.02 & 78.47$\pm$1.04 & 77.88$\pm$0.90 \\
10 & 72.54$\pm$0.01 & 71.12$\pm$0.02 & 79.57$\pm$0.05 & 78.52$\pm$0.13 & 68.78$\pm$0.01 & 63.52$\pm$0.02 & 75.67$\pm$1.30 & 74.84$\pm$0.59 \\
20 & 76.59$\pm$0.01 & 75.46$\pm$0.02 & 78.37$\pm$0.01 & 77.16$\pm$0.05 & 71.63$\pm$0.01 & 68.85$\pm$0.01 & 76.64$\pm$2.51 & 76.00$\pm$1.70 \\
\midrule

\multicolumn{9}{l}{\textbf{Relative Sparsity $\mathbf{s}=50\%$}}\\
2  & 74.77$\pm$0.01 & 73.50$\pm$0.01 & 80.18$\pm$0.18 & 79.26$\pm$0.52 & 73.27$\pm$0.07 & 71.43$\pm$0.04 & 72.53$\pm$4.98 & 71.46$\pm$3.88 \\
5  & 75.51$\pm$0.02 & 74.09$\pm$0.01 & 79.83$\pm$0.06 & 78.88$\pm$0.24 & 75.53$\pm$0.03 & 74.26$\pm$0.01 & 75.45$\pm$2.53 & 75.46$\pm$1.75 \\
10 & 72.58$\pm$0.01 & 70.89$\pm$0.00 & 80.68$\pm$0.02 & 79.80$\pm$0.10 & 71.29$\pm$0.02 & 68.47$\pm$0.01 & 73.61$\pm$0.25 & 71.36$\pm$1.03 \\
20 & 76.52$\pm$0.00 & 75.53$\pm$0.00 & 80.61$\pm$0.02 & 79.85$\pm$0.03 & 72.92$\pm$0.01 & 71.15$\pm$0.04 & 79.94$\pm$0.75 & 79.08$\pm$0.37 \\
\bottomrule
\end{tabular}


==> tables/US_UK_f1.tex <==
% Requires in preamble:
% \usepackage{booktabs}
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c}
\toprule
& \multicolumn{2}{c}{\textbf{Acoustic NACs}} 
& \multicolumn{2}{c}{\textbf{Phonetic NACs}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\textbf{$\frac{D_\text{z}}{D_\text{d}}$}
& \textbf{EnCodec} 
& \textbf{DAC}
& \textbf{Mimi} 
& \textbf{SpeechTokenizer} \\
\midrule

\multicolumn{5}{l}{\textbf{Reference}}\\
1  & 83.72$\pm$0.02 & 83.53$\pm$0.03 & 90.59$\pm$0.00 & 93.45$\pm$0.01 \\
\midrule

\multicolumn{5}{l}{\textbf{Relative Sparsity $\mathbf{s}=5\%$}}\\
2  & 67.91$\pm$0.04 & 79.45$\pm$0.14 & 61.35$\pm$0.00 & 74.60$\pm$0.50 \\
5  & 64.62$\pm$0.26 & 79.51$\pm$0.02 & 75.47$\pm$0.00 & 70.46$\pm$0.25 \\
10 & 64.62$\pm$0.07 & 79.69$\pm$0.02 & 71.81$\pm$0.00 & 73.67$\pm$1.09 \\
20 & 67.97$\pm$0.02 & 80.79$\pm$0.03 & 73.11$\pm$0.00 & 72.18$\pm$0.08 \\
\midrule

\multicolumn{5}{l}{\textbf{Relative Sparsity $\mathbf{s}=10\%$}}\\
2  & 64.86$\pm$0.18 & 79.56$\pm$0.04 & 70.09$\pm$0.01 & 78.97$\pm$0.50 \\
5  & 73.22$\pm$0.04 & 80.16$\pm$0.02 & 69.45$\pm$0.00 & 69.60$\pm$0.11 \\
10 & 69.13$\pm$0.05 & 78.77$\pm$0.08 & 70.19$\pm$0.00 & 74.11$\pm$0.05 \\
20 & 68.68$\pm$0.01 & 78.59$\pm$0.13 & 73.54$\pm$0.00 & 76.95$\pm$0.43 \\
\midrule

\multicolumn{5}{l}{\textbf{Relative Sparsity $\mathbf{s}=25\%$}}\\
2  & 78.38$\pm$0.01 & 77.98$\pm$0.06 & 68.60$\pm$0.05 & 80.84$\pm$0.23 \\
5  & 71.58$\pm$0.01 & 79.24$\pm$0.11 & 70.93$\pm$0.02 & 77.88$\pm$0.90 \\
10 & 71.12$\pm$0.02 & 78.52$\pm$0.13 & 63.52$\pm$0.02 & 74.84$\pm$0.59 \\
20 & 75.46$\pm$0.02 & 77.16$\pm$0.05 & 68.85$\pm$0.01 & 76.00$\pm$1.70 \\
\midrule

\multicolumn{5}{l}{\textbf{Relative Sparsity $\mathbf{s}=50\%$}}\\
2  & 73.50$\pm$0.01 & 79.26$\pm$0.52 & 71.43$\pm$0.04 & 71.46$\pm$3.88 \\
5  & 74.09$\pm$0.01 & 78.88$\pm$0.24 & 74.26$\pm$0.01 & 75.46$\pm$1.75 \\
10 & 70.89$\pm$0.00 & 79.80$\pm$0.10 & 68.47$\pm$0.01 & 71.36$\pm$1.03 \\
20 & 75.53$\pm$0.00 & 79.85$\pm$0.03 & 71.15$\pm$0.04 & 79.08$\pm$0.37 \\
\bottomrule
\end{tabular}
}

==> tables/reference_table.tex <==
% Requires in preamble:
% \usepackage{booktabs}

\resizebox{\linewidth}{!}{
\begin{tabular}{l c c c c}
\toprule

& \shortstack{\textbf{EnCodec}\\ \textbf{1.5} / \textbf{6} / \textbf{12 kbps} } 
& \makecell{\textbf{DAC}}
& \makecell{\textbf{Mimi}}
& \shortstack{\textbf{Speech}\\\textbf{Tokenizer}} \\
\midrule

% \multicolumn{5}{l}{\textbf{US vs UK}} \\
% \midrule
\textbf{US vs.\ UK}  
& 0.811 / 0.802 / 0.802
& 0.800
& 0.888 
& \textbf{0.924}\\

\midrule
% \multicolumn{5}{l}{\textbf{US vs Others}} \\
% \midrule

\makecell[l]{\textbf{US vs.}\\\textbf{Non-US-UK}}
& 0.572 / 0.609 / 0.620
& 0.613
& 0.757
& \textbf{0.760} \\

\bottomrule
\end{tabular}
}
